Cosmology Intertwined: A Review of the Particle Physics, Astrophysics, and Cosmology Associated with the Cosmological Tensions and Anomalies

In this paper we will list a few important goals that need to be addressed in the next decade, also taking into account the current discordances between the different cosmological probes, such as the disagreement in the value of the Hubble constant $H_0$, the $\sigma_8$--$S_8$ tension, and other less statistically significant anomalies. While these discordances can still be in part the result of systematic errors, their persistence after several years of accurate analysis strongly hints at cracks in the standard cosmological scenario and the necessity for new physics or generalisations beyond the standard model. In this paper, we focus on the $5.0\,\sigma$ tension between the {\it Planck} CMB estimate of the Hubble constant $H_0$ and the SH0ES collaboration measurements. After showing the $H_0$ evaluations made from different teams using different methods and geometric calibrations, we list a few interesting new physics models that could alleviate this tension and discuss how the next decade's experiments will be crucial. Moreover, we focus on the tension of the {\it Planck} CMB data with weak lensing measurements and redshift surveys, about the value of the matter energy density $\Omega_m$, and the amplitude or rate of the growth of structure ($\sigma_8,f\sigma_8$). We list a few interesting models proposed for alleviating this tension, and we discuss the importance of trying to fit a full array of data with a single model and not just one parameter at a time. Additionally, we present a wide range of other less discussed anomalies at a statistical significance level lower than the $H_0$--$S_8$ tensions which may also constitute hints towards new physics, and we discuss possible generic theoretical approaches that can collectively explain the non-standard nature of these signals.[Abridged]

==> Cosmology Intertwined White Paper/AuthorsListFeb2021.tex <==
\author{Elcio Abdalla}
\affiliation{Instituto de F\'isica, Universidade de S\~ao Paulo - C.P. 66318, CEP: 05315-970, S\~ao Paulo, Brazil}

\author{Guillermo Franco Abell\'an}
\affiliation{
 Laboratoire Univers \& Particules de Montpellier (LUPM), Universit\'e de Montpellier (UMR-5299) \\ Place Eug{\`e}ne Bataillon, F-34095 Montpellier Cedex 05, France 
}

\author{Amin Aboubrahim}
\affiliation{Institut f\"ur Theoretische Physik, Westf\"alische Wilhelms-Universit\"at M\"unster, Wilhelm-Klemm-Stra{\ss}e 9, 48149 M\"unster, Germany}


\author{Adriano Agnello}
\affiliation{DARK, Niels Bohr Institute, University of Copenhagen, Jagtvej 128, 2200 Copenhagen, Denmark}

\author{\"{O}zg\"{u}r Akarsu}
\affiliation{Department of Physics, Istanbul Technical University, Maslak 34469 Istanbul, Turkey}

\author{Yashar Akrami}
\affiliation{CERCA/ISO, Department of Physics, Case Western Reserve University, 10900 Euclid Avenue, Cleveland, OH 44106, USA}
\affiliation{Astrophysics Group \& Imperial Centre for Inference and Cosmology,
Department of Physics, Imperial College London, Blackett Laboratory,
Prince Consort Road, London SW7 2AZ, United Kingdom}
\affiliation{Laboratoire de Physique de l'\'Ecole Normale Sup\'erieure, ENS, Universit\'e PSL, CNRS, Sorbonne Universit\'e, Universit\'e de Paris, F-75005 Paris, France}
\affiliation{Observatoire de Paris, Universit\'e PSL, Sorbonne Universit\'e, LERMA, 75014 Paris, France}

\author{George Alestas}
\affiliation{Department of Physics, University of Ioannina, GR-45110, Ioannina, Greece}

\author{Daniel Aloni}
\affiliation{Physics Department, Boston University, Boston, MA 02215, USA}

\author{Luca Amendola}
\affiliation{Institute of Theoretical Physics, Heidelberg University,
Philosophenweg 16, 69120 Heidelberg, Germany}

\author{Luis A. Anchordoqui}
\affiliation{Department of Physics and Astronomy,  Lehman College, City University of New York, NY 10468, USA}
\affiliation{Department of Physics, Graduate Center, City University of New York,  NY 10016, USA}
\affiliation{Department of Astrophysics, American Museum of Natural History, NY 10024, USA}

\author{Richard I. Anderson}
\affiliation{Institute of Physics, Laboratory of Astrophysics,
\'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Observatoire de Sauverny, 1290 Versoix, Switzerland}

\author{Nikki Arendse}
\affiliation{Oskar Klein Centre, Department of Physics, Stockholm University, SE-106 91 Stockholm, Sweden}

\author{Marika Asgari}
\affiliation{E.A Milne Centre, University of Hull, Cottingham Road, Hull, HU6 7RX, United Kingdom}
\affiliation{Institute for Astronomy, University of Edinburgh, Royal Observatory, Blackford Hill, Edinburgh, EH9 3HJ, United Kingdom}


\author{Mario Ballardini}
\affiliation{Dipartimento di Fisica e Astronomia, Universit{\`a} di Bologna, viale Berti Pichat 6/2, 40127 Bologna, Italy}
\affiliation{INAF/OAS Bologna, via Piero Gobetti 101, I-40129 Bologna, Italy}
\affiliation{INFN, Sezione di Bologna, viale Berti Pichat 6/2, 40127 Bologna, Italy}
\affiliation{Department of Physics \& Astronomy, University of the Western Cape, Cape Town 7535, South Africa}

\author{Vernon Barger}
\affiliation{Department of Physics, University of Wisconsin, Madison, WI 53706, USA}

\author{Spyros Basilakos}
\affiliation{Academy of Athens, Research Center for Astronomy and Applied Mathematics, Soranou Efesiou 4, 11527, Athens, Greece} 
\affiliation{National Observatory of Athens, Lofos Nymfon, 11852 Athens, Greece}

\author{Ronaldo C. Batista}
\affiliation{Escola de Ci\^encias e Tecnologia, Universidade Federal do Rio Grande do Norte,  59078-970, Natal, RN, Brazil}

\author{Elia S. Battistelli}
\affiliation{Dipartimento di Fisica, Sapienza Universit{\`a} di Roma, P.le A. Moro 2, I-00185, Roma, Italy} 
\affiliation{INFN Sezione di Roma, P.le A. Moro 2, I-00185, Roma, Italy}

\author{Richard Battye}
\affiliation{Jodrell Bank Centre for Astrophysics, University of Manchester, Oxford Road, Manchester M13 9PL, United Kingdom} 


\author{Micol Benetti}
\affiliation{Scuola Superiore Meridionale, Largo S. Marcellino 10, I-80138, Napoli, Italy} 
\affiliation{Istituto Nazionale di Fisica Nucleare (INFN) Sezione di Napoli, Complesso Universitario di Monte Sant'Angelo,  Edificio G,
  Via Cinthia, I-80126, Napoli, Italy}

\author{David Benisty}
\affiliation{DAMTP, Centre for Mathematical Sciences, University of Cambridge, Wilberforce Road, Cambridge CB3 0WA, United Kingdom}
\affiliation{Kavli Institute of Cosmology (KICC), University of Cambridge, Madingley Road, Cambridge, CB3 0HA, United Kingdom} 
\affiliation{Queens’ College, Cambridge, CB3 9ET, United Kingdom} 


\author{Asher Berlin}
\affiliation{Theoretical Physics Department, Fermilab, P.O. Box 500, Batavia, IL 60510, USA}

\author{Paolo de Bernardis}
\affiliation{Dipartimento di Fisica, Sapienza Universit{\`a} di Roma, P.le A. Moro 2, I-00185, Roma, Italy} 
\affiliation{INFN Sezione di Roma, P.le A. Moro 2, I-00185, Roma, Italy} 

\author{Emanuele Berti}
\affiliation{Department of Physics and Astronomy, Johns Hopkins University, Baltimore, Maryland 21218, USA}

\author{Bohdan Bidenko}
\affiliation{Kapteyn Astronomical Institute, University of Groningen, P.O. Box 9000,
9700 AA Groningen, The Netherlands}
\affiliation{Van Swinderen Institute for Particle Physics and Gravity, University of Groningen, Nijenborgh 4, 9747 AG Groningen, The Netherlands}

\author{Simon Birrer}
\affiliation{Kavli Institute for Particle Astrophysics and Cosmology and Department of Physics, Stanford University, Stanford, CA 94305, USA}

\author{John P. Blakeslee}
\affiliation{NSF's National Optical-Infrared Astronomy Research Laboratory (NOIRLab), Tucson, AZ 85719, USA}

\author{Kimberly K.~Boddy}
\affiliation{Department of Physics, The University of Texas at Austin, Austin, TX 78712}

\author{Clecio R. Bom}
\affiliation{Centro Brasileiro de Pesquisas F\'isicas, Rua Dr. Xavier Sigaud 150, 22290-180 Rio de Janeiro, RJ, Brazil}
\affiliation{Centro Federal de Educa\c{c}\~{a}o Tecnol\'{o}gica Celso Suckow da Fonseca, Rodovia M\'{a}rcio Covas, lote J2, quadra J - Itagua\'{i} (Brazil)}

\author{Alexander Bonilla}
\affiliation{Departamento de F\'isica, Universidade Federal de Juiz de Fora, 36036-330, Juiz de Fora, MG, Brazil}

\author{Nicola Borghi}
\affiliation{Dipartimento di Fisica e Astronomia ``Augusto Righi'', Alma Mater Studiorum Universit\`{a} di Bologna, via Piero Gobetti 93/2, I-40129 Bologna, Italy}
\affiliation{INAF - Osservatorio di Astrofisica e Scienza dello Spazio di Bologna, via Piero Gobetti 93/3, I-40129 Bologna, Italy}

\author{Fran\c{c}ois R. Bouchet}
\affiliation{Institut d'Astrophysique de Paris, CNRS \& Sorbonne University\\ 98 bis Boulevard Arago, 75014, Paris, France}

\author{Matteo Braglia}
\affiliation{Instituto de Fisica Teorica, Universidad Autonoma de Madrid, Madrid, 28049, Spain}
\affiliation{INAF/OAS Bologna, via Piero Gobetti 101, I-40129 Bologna, Italy}

\author{Thomas~Buchert}
\affiliation{Univ Lyon, Ens de Lyon, Univ Lyon1, CNRS, Centre de Recherche Astrophysique de Lyon UMR5574, F--69007, Lyon, France}

\author{Elizabeth Buckley-Geer}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}

\author{Erminia Calabrese}
\affiliation{School of Physics and Astronomy, Cardiff University, The Parade, Cardiff, CF24 3AA, United Kingdom}

\author{Robert R. Caldwell}
\affiliation{Department of Physics \& Astronomy, Dartmouth College, 6127 Wilder Laboratory, Hanover, New Hampshire 03755 USA}

\author{David Camarena}
\affiliation{PPGCosmo, Universidade Federal do Esp{\'i}rito Santo, 29075-910, Vit{\'o}ria, ES, Brazil}

\author{Salvatore Capozziello}
\affiliation{Dipartimento di Fisica ``E. Pancini'', Universit{\`a} degli Studi di Napoli ``Federico II'', Complesso Universitario di Monte S. Angelo, Ed. G, Via Cinthia, I-80126, Napoli, Italy} 
\affiliation{Scuola Superiore Meridionale, Largo S. Marcellino 10, I-80138, Napoli, Italy}

\author{Stefano Casertano}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}

\author{Angela Chen}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}
\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (Kavli IPMU, WPI), Kashiwanoha, Chiba, 277-8583, Japan}

\author{Geoff C.-F. Chen}
\affiliation{Department of Physics and Astronomy, University of California, Los Angeles CA 90095, USA}

\author{Hsin-Yu Chen}
\affiliation{Department of Physics and Kavli Institute for Astrophysics and Space Research, Massachusetts Institute of Technology, 77 Massachusetts Ave, Cambridge, MA 02139, USA}

\author{Jens Chluba}
\affiliation{Jodrell Bank Centre for Astrophysics, University of Manchester, Oxford Road, Manchester M13 9PL, United Kingdom}

\author{Anton Chudaykin}
\affiliation{Department of Physics \& Astronomy, McMaster University, 1280 Main Street West, Hamilton, ON L8S 4M1, Canada}

\author{Michele Cicoli}
\affiliation{Dipartimento di Fisica e Astronomia, Universit{\`a} di Bologna, viale Berti Pichat 6/2, 40127 Bologna, Italy}
\affiliation{INFN, Sezione di Bologna, viale Berti Pichat 6/2, 40127 Bologna, Italy}

\author{Craig J. Copi}
\affiliation{CERCA/ISO, Department of Physics, Case Western Reserve University, 10900 Euclid Avenue, Cleveland, OH 44106, USA}

\author{Fred Courbin}
\affiliation{Institute of Physics, Laboratory of Astrophysics, \'Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Observatoire de Sauverny, 1290 Versoix, Switzerland}

\author{Francis-Yan Cyr-Racine}
\affiliation{Department of Physics and Astronomy, University of New Mexico, Albuquerque, NM 87106, USA}

\author{Bo\. zena Czerny}
\affiliation{Center for Theoretical Physics, Polish Academy of Sciences, Al. Lotnikow 32/46, 02-668 Warsaw, Poland}
\author{Maria Dainotti}
\affiliation{National Astronomical Observatory of Japan, 2 Chome-21-1 Osawa, Mitaka, Tokyo 181-8588, Japan}
\affiliation{The Graduate University for Advanced Studies, SOKENDAI, Shonankokusaimura, Hayama, Miura District, Kanagawa 240-0193, Japan}
\affiliation{Space Science Institute, Boulder, CO, USA}

\author{Guido D'Amico}
\affiliation{Dipartimento di Scienze Matematiche, Fisiche e Informatiche, Universit{\`a} di Parma, Parco Area delle Scienze 7/A, 43124 Parma}
\affiliation{INFN Gruppo Collegato di Parma, 43124 Parma, Italy}

\author{Anne-Christine Davis}
\affiliation{DAMTP, Centre for Mathematical Sciences, University of Cambridge, Wilberforce Road, Cambridge CB3 0WA, United Kingdom}
\affiliation{Kavli Institute of Cosmology (KICC), University of Cambridge, Madingley Road, Cambridge, CB3 0HA, United Kingdom} 

\author{Javier de Cruz P\'erez}
\affiliation{Department of Physics, Kansas State University, 116 Cardwell Hall, Manhattan, KS 66502 USA}

\author{Jaume de Haro}
\affiliation{Departament de Matem\' {a}tica Aplicada, Universitat Polit\`{e}cnica de Catalunya, Diagonal 647, 08028 Barcelona, Spain. }

\author{Jacques Delabrouille}
\affiliation{CNRS-UCB International Research Laboratory, Centre Pierre Bin{\'e}truy, IRL2007, CPB-IN2P3, Berkeley, USA}
\affiliation{Laboratoire Astroparticule et Cosmologie (APC), CNRS/IN2P3, Universit\'e Paris Diderot, 75205 Paris Cedex 13, France}
\affiliation{IRFU, CEA, Universit\'e Paris Saclay, 91191 Gif-sur-Yvette, France}
\affiliation{Department of Astronomy, School of Physical Sciences, University of Science and Technology of China, Hefei, Anhui 230026, P.\ R.\ China} 

\author{Peter B.~Denton}
\affiliation{High Energy Theory Group, Physics Department, Brookhaven National Laboratory, Upton, NY 11973, USA}

\author{Suhail Dhawan}
\affiliation{Institute of Astronomy and Kavli Institute for Cosmology, University of Cambridge, Madingley Road, Cambridge CB3 0HA, UK}

\author{Keith R. Dienes}
\affiliation{Department of Physics, University of Arizona, Tucson, AZ 85721, USA} 
\affiliation{Department of Physics, University of Maryland, College Park, MD 20742, USA}


\author{Eleonora Di Valentino}
\email{Corresponding author (e.divalentino@sheffield.ac.uk)}
\affiliation{School of Mathematics and Statistics, University of Sheffield, Hounsfield Road, Sheffield S3 7RH, United Kingdom}



\author{Pu Du}
\affiliation{Key Laboratory for Particle Astrophysics, Institute of High Energy Physics, Chinese Academy of Sciences, 19B Yuquan Road, Beijing 100049, P.\ R.\ China}

\author{Dominique Eckert}
\affiliation{Department of Astronomy, University of Geneva, Ch. d'Ecogia 16, CH-1290 Versoix, Switzerland}


\author{Celia Escamilla-Rivera}
\affiliation{Instituto de Ciencias Nucleares, Universidad Nacional Aut\'onoma de M\'exico, 
Circuito Exterior C.U., A.P. 70-543, M\'exico D.F. 04510, M\'exico}

\author{Agn\`es Fert\'e}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Drive, Pasadena, CA, 91109, USA}

\author{Fabio Finelli}
\affiliation{Osservatorio di Astrofisica e Scienza dello Spazio di Bologna \& Istituto Nazionale di Astrofisica, via Gobetti 101, I-40129 Bologna, Italy}
\affiliation{INFN, Sezione di Bologna, viale Berti Pichat 6/2, 40127 Bologna, Italy}

\author{Pablo Fosalba}
\affiliation{Institute of Space Sciences (ICE, CSIC), Campus UAB, Carrer de Can Magrans, s/n, 08193 Barcelona, Spain}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), Carrer Gran Capit\`a 2-4, 08193 Barcelona, Spain}

\author{Wendy L. Freedman}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}

\author{Noemi Frusciante}
\affiliation{Instituto de Astrof\'isica e Ci\^encias do Espa\c{c}o, Faculdade de Ci\^encias da Universidade de Lisboa,  
\\ Edificio C8, Campo Grande, P-1749016, Lisboa, Portugal}

\author{Enrique Gazta\~{n}aga}
\affiliation{Institute of Space Sciences (ICE, CSIC), Campus UAB, Carrer de Can Magrans, s/n, 08193 Barcelona, Spain}
\affiliation{Institut d'Estudis Espacials de Catalunya (IEEC), Carrer Gran Capit\`a 2-4, 08193 Barcelona, Spain}

\author{William Giar\`e}
\affiliation{Galileo Galilei Institute for theoretical physics, National Centre of Advanced Studies of INFN \\ Largo Enrico Fermi 2,  I-50125, Firenze, Italy}
\affiliation{INFN Sezione di Roma, P.le A. Moro 2, I-00185, Roma, Italy} 

\author{Elena Giusarma}
\affiliation{Department of Physics, Michigan Technological University, Houghton, MI 49931, USA}

\author{Adri\`a G\'omez-Valent}
\affiliation{Dipartamento di Fisica and INFN Sezione di Roma Tor Vergata, via della Ricerca Scientifica 1, 00133 Roma, Italy}

\author{Will Handley}
\affiliation{Astrophysics Group, Cavendish Laboratory, J.~J.~Thomson Avenue, Cambridge, CB3~0HE, United Kingdom}
\affiliation{Kavli Institute for Cosmology, Madingley Road, Cambridge, CB3~0HA, United Kingdom}

\author{Ian Harrison}
\affiliation{School of Physics and Astronomy, Cardiff University, Cardiff, CF24 3AA, United Kingdom}

\author{Luke Hart}
\affiliation{Jodrell Bank Centre for Astrophysics, University of Manchester, Oxford Road, Manchester M13 9PL, United Kingdom}

\author{Dhiraj Kumar Hazra}
\affiliation{The Institute of Mathematical Sciences, HBNI, CIT Campus, Chennai 600113, India}


\author{Alan Heavens}
\affiliation{Astrophysics Group \& Imperial Centre for Inference and Cosmology,
Department of Physics, Imperial College London, Blackett Laboratory,
Prince Consort Road, London SW7 2AZ, United Kingdom}

\author{Asta~Heinesen}
\affiliation{Univ Lyon, Ens de Lyon, Univ Lyon1, CNRS, Centre de Recherche Astrophysique de Lyon UMR5574, F--69007, Lyon, France}


\author{Hendrik Hildebrandt}
\affiliation{Ruhr University Bochum, Faculty of Physics and Astronomy, Astronomical Institute (AIRUB), German Centre for Cosmological Lensing, 44780 Bochum, Germany}

\author{J.~Colin Hill}
\affiliation{Department of Physics, Columbia University, New York, NY 10027, USA}
\affiliation{Center for Computational Astrophysics, Flatiron Institute, New York, NY 10010, USA}

\author{Natalie B. Hogg}
\affiliation{Instituto de F\'{i}sica Te\'{o}rica UAM-CSIC, C/ Nicol\'{a}s Cabrera 13-15,  Universidad Aut\'{o}noma de Madrid, Cantoblanco, Madrid 28049, Spain}

\author{Daniel E. Holz}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\affiliation{Department of Physics and Enrico Fermi Institute, University of Chicago, Chicago IL 60637 USA}

\author{Deanna C. Hooper}
\affiliation{Department of Physics and Helsinki Institute of Physics, PL 64, FI-00014 University of Helsinki, Finland}

\author{Nikoo Hosseininejad}
\affiliation{Department of Physics, Shahid Beheshti University, 1983969411, Tehran, Iran}

\author{Dragan Huterer}
\affiliation{Department of Physics, University of Michigan, 450 Church St, Ann Arbor, MI 48109-1040, USA}
\affiliation{Leinweber Center for Theoretical Physics, University of Michigan, 450 Church St, Ann Arbor, MI 48109-1040, USA}


\author{Mustapha Ishak}
\affiliation{Department of Physics, The University of Texas at Dallas, Richardson, Texas 75080, USA}

\author{Mikhail M. Ivanov}
% \affiliation{Center for Cosmology and Particle Physics, Department of Physics, New York University,\\
% New York, NY 10003, USA}
\affiliation{School of Natural Sciences, Institute for Advanced Study, 1 Einstein Drive, Princeton, NJ 08540, USA}


\author{Andrew H. Jaffe}
\affiliation{Astrophysics Group \& Imperial Centre for Inference and Cosmology,
Department of Physics, Imperial College London, Blackett Laboratory,
Prince Consort Road, London SW7 2AZ, United Kingdom}

\author{In Sung Jang}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}


\author{Karsten Jedamzik} 
\affiliation{Laboratoire de Univers et Particules de Montpellier, UMR5299-CNRS, Universite de Montpellier, 34095 Montpellier, France}

\author{Raul Jimenez}
\affiliation{ICCUB, University of Barcelona, Marti i Franques 1, Barcelona, 08028, Spain}
\affiliation{ICREA, Pg. Lluis Companys 23, Barcelona, 08010, Spain} 

\author{Melissa Joseph}
\affiliation{Physics Department, Boston University, Boston, MA 02215, USA}

\author{Shahab Joudaki}
\affiliation{Waterloo Centre for Astrophysics, University of Waterloo, 200 University Ave W, Waterloo, ON N2L 3G1, Canada}
\affiliation{Department of Physics and Astronomy, University of Waterloo, 200 University Ave W, Waterloo, ON N2L 3G1, Canada}

\author{Marc Kamionkowski}
\affiliation{Department of Physics and Astronomy, Johns Hopkins University, Baltimore, Maryland 21218, USA}

\author{Tanvi Karwal}
\affiliation{Center for Particle Cosmology, Department of Physics and Astronomy, University of Pennsylvania, Philadelphia PA 19104, USA}

\author{Lavrentios Kazantzidis}
\affiliation{Department of Physics, University of Ioannina, GR-45110, Ioannina, Greece}

\author{Ryan E. Keeley}
\affiliation{Department of Physics, University of California Merced, 5200 North Lake Road, Merced, CA 95343, USA}

\author{Michael Klasen}
\affiliation{Institut f\"ur Theoretische Physik, Westf\"alische Wilhelms-Universit\"at M\"unster, Wilhelm-Klemm-Stra{\ss}e 9, 48149 M\"unster, Germany}

\author{Eiichiro Komatsu}
\affiliation{Max Planck Institute for Astrophysics, Karl-Schwarzschild-Str. 1, D-85748 Garching, Germany} 
\affiliation{Kavli Institute for the Physics  Mathematics of the Universe (Kavli IPMU, WPI),
Todai Institutes for Advanced Study, The University of Tokyo, Kashiwa 277-8583, Japan}

\author{L\'eon V.E. Koopmans}
\affiliation{Kapteyn Astronomical Institute, University of Groningen, P.O. Box 800, 9700AV Groningen, The Netherlands}

\author{Suresh Kumar}
\affiliation{Department of Mathematics, Indira Gandhi University, Meerpur, Haryana-122502, India}

\author{Luca Lamagna}
\affiliation{Dipartimento di Fisica, Sapienza Universit{\`a} di Roma, P.le A. Moro 2, I-00185, Roma, Italy}
\affiliation{INFN Sezione di Roma, P.le A. Moro 2, I-00185, Roma, Italy}


\author{Ruth Lazkoz}
\affiliation{Department of Physics, University of the Basque Country UPV/EHU, P.O. Box 644, 48080 Bilbao, Spain}

\author{Chung-Chi Lee}
\affiliation{Clare Hall, University of Cambridge, Herschel Rd, Cambridge CB3 9AL, United Kingdom}

\author{Julien Lesgourgues}
\affiliation{Institute for Theoretical Particle Physics and Cosmology (TTK), RWTH Aachen University, D-52056 Aachen, Germany}

\author{Jackson Levi Said}
\affiliation{Institute of Space Sciences and Astronomy, University of Malta, Msida, MSD 2080, Malta}
\affiliation{Department of Physics, University of Malta, Msida, MSD 2080, Malta}

\author{Tiffany R. Lewis}
\affiliation{Astroparticle Physics Laboratory, NASA Goddard Space Flight Center, Greenbelt, MD, USA}
%\affiliation{NASA Postdoctoral Program Fellow}

\author{Benjamin L'Huillier}
\affiliation{Department of Physics and Astronomy, Sejong University, Seoul 05006, Korea}

\author{Matteo Lucca}
\affiliation{Service de Physique Th\'eorique, Universit\'e Libre de Bruxelles, Boulevard du Triomphe, CP225, 1050 Brussels, Belgium}

\author{Roy Maartens}
\affiliation{Department of Physics \& Astronomy, University of the Western Cape, Cape Town 7535, South Africa}
\affiliation{Institute of Cosmology \& Gravitation, University of Portsmouth, Portsmouth PO1 3FX, United Kingdom}
\affiliation{National Institute for Theoretical \& Computational Sciences (NITheCS), Pretoria 2600, South Africa}

\author{Lucas~M.~Macri}
\affiliation{George P. and Cynthia W. Mitchell Institute for Fundamental Physics \& Astronomy,\\ Department of Physics \& Astronomy, Texas A\&M University, College Station, TX, USA}

\author{Danny Marfatia}
\affiliation{Department of Physics and Astronomy, University of Hawaii, Honolulu, HI 96822, USA}

\author{Valerio Marra}
\affiliation{N{\'u}cleo de Astrof{\'i}sica e Cosmologia (Cosmo-ufes) \& Departamento de F{\'i}sica, Universidade Federal do Esp{\'i}rito Santo, 29075-910, Vit{\'o}ria, ES, Brazil}
\affiliation{INAF -- Osservatorio Astronomico di Trieste, via Tiepolo 11, 34131 Trieste, Italy}
\affiliation{IFPU -- Institute for Fundamental Physics of the Universe, via Beirut 2, 34151, Trieste, Italy}

\author{Carlos J. A. P. Martins}
\affiliation{Centro de Astrof\'{\i}sica da Universidade do Porto, Rua das Estrelas, 4150-762 Porto, Portugal}
\affiliation{Instituto de Astrof\'{\i}sica e Ci\^encias do Espa\c co, Universidade do Porto, Rua das Estrelas, 4150-762 Porto, Portugal}

\author{Silvia Masi}
\affiliation{Dipartimento di Fisica, Sapienza Universit{\`a} di Roma, P.le A. Moro 2, I-00185, Roma, Italy} 
\affiliation{INFN Sezione di Roma, P.le A. Moro 2, I-00185, Roma, Italy} 

\author{Sabino Matarrese}
\affiliation{Dipartimento di Fisica e Astronomia ``Galileo Galilei", Universit{\`a} degli Studi di Padova, via F. Marzolo 8, I-35131, Padova, Italy}
\affiliation{INFN, Sezione di Padova, via F. Marzolo 8, I-35131, Padova, Italy}
\affiliation{INAF-Osservatorio Astronomico di Padova, Vicolo dell'Osservatorio 5, I-35122 Padova, Italy}
\affiliation{Gran Sasso Science Institute, Viale F. Crispi 7, I-67100 L'Aquila, Italy}

\author{Arindam Mazumdar}
\affiliation{Department of Physics, Indian Institute of Technology Kharagpur, Kharagpur - 721302, India}

\author{Alessandro Melchiorri}
\affiliation{Dipartimento di Fisica, Sapienza Universit{\`a} di Roma, P.le A. Moro 2, I-00185, Roma, Italy} 
\affiliation{INFN Sezione di Roma, P.le A. Moro 2, I-00185, Roma, Italy} 

\author{Olga Mena}
\affiliation{Instituto de F{\'i}sica Corpuscular (CSIC-Universitat de Val{\`e}ncia), Paterna, Spain}

\author{Laura Mersini-Houghton}
\affiliation{Department of Physics and Astronomy, University of North Carolina at Chapel Hill, NC, 27599, USA}

\author{James Mertens}
\affiliation{Department of Physics and McDonnell Center for the Space Sciences,
Washington University, St. Louis, MO 63130, USA}

\author{Dinko Milakovi{\'c}}
\affiliation{IFPU -- Institute for Fundamental Physics of the Universe, via Beirut 2, 34151, Trieste, Italy}
\affiliation{INAF -- Osservatorio Astronomico di Trieste, via Tiepolo 11, 34131 Trieste, Italy}
\affiliation{INFN, Sezione di Trieste, Via Bonomea 265, 34136 Trieste, Italy}

\author{Yuto Minami}
\affiliation{Research Center for Nuclear Physics, Osaka University, Ibaraki, Osaka, 567-0047 Japan}

\author{Vivian Miranda}
\affiliation{C. N. Yang Institute for Theoretical Physics, Stony Brook University, Stony Brook, NY 11794} 
 
\author{Cristian Moreno-Pulido}
\affiliation{Departament de F\'\i sica Qu\`antica i Astrof\'\i sica and Institute of Cosmos Sciences, Universitat de Barcelona, Av. Diagonal 647, E-08028 Barcelona, Catalonia, Spain}

\author{Michele Moresco}
\affiliation{Dipartimento di Fisica e Astronomia ``Augusto Righi'', Alma Mater Studiorum Universit\`{a} di Bologna, via Piero Gobetti 93/2, I-40129 Bologna, Italy}
\affiliation{INAF - Osservatorio di Astrofisica e Scienza dello Spazio di Bologna, via Piero Gobetti 93/3, I-40129 Bologna, Italy}

\author{David F. Mota}
\affiliation{Institute of Theoretical Astrophysics, University of Oslo, 0315 Oslo, Norway}

\author{Emil Mottola}
\affiliation{Department of Physics and Astronomy, University of New Mexico, Albuquerque, NM 87106, USA}

\author{Simone Mozzon}
\affiliation{Institute of Cosmology and Gravitation, University of Portsmouth,
Portsmouth, PO13FX, United Kingdom}

\author{Jessica Muir}
\affiliation{Perimeter Institute for Theoretical Physics, 31 Caroline Street N., Waterloo, Ontario, N2L 2Y5, Canada}

\author{Ankan Mukherjee}
\affiliation{Centre for Theoretical Physics, Jamia Millia Islamia, New Delhi, 110025, India}

\author{Suvodip Mukherjee}
\affiliation{Perimeter Institute for Theoretical Physics, 31 Caroline Street N., Waterloo, Ontario, N2L 2Y5, Canada}

\author{Pavel Naselsky}
\affiliation{Niels Bohr Institute, Blegdamsvej 17, Copenhagen, Denmark}

\author{Pran Nath}
\affiliation{Department of Physics, Northeastern University, Boston, MA 02115, USA}

\author{Savvas Nesseris}
\affiliation{Instituto de F\'{i}sica Te\'{o}rica UAM-CSIC, C/ Nicol\'{a}s Cabrera 13-15,  Universidad Aut\'{o}noma de Madrid, Cantoblanco, Madrid 28049, Spain}

\author{Florian Niedermann}
\affiliation{Nordita, KTH Royal Institute of Technology and Stockholm University, Hannes Alfv\'ens v\"ag 12, SE-106 91 Stockholm, Sweden}

\author{Alessio Notari}
\affiliation{Departament de F\'isica Qu\`antica i Astrofis\'ica \& Institut de Ci\`encies del Cosmos (ICCUB), Universitat de Barcelona, Mart\'i i Franqu\`es 1, 08028 Barcelona, Spain}

\author{Rafael C. Nunes}
\affiliation{Divis\~ao de Astrof\'isica, Instituto Nacional de Pesquisas Espaciais, Avenida dos Astronautas 1758, S\~ao Jos\'e dos Campos, 12227-010, SP, Brazil}

\author{Eoin \'O Colg\'ain}
\affiliation{Center for Quantum Spacetime, Sogang University, Seoul 121-742, Korea}
\affiliation{Department of Physics, Sogang University, Seoul 121-742, Korea}

\author{Kayla A. Owens}
\affiliation{Department of Astronomy and Astrophysics, University of Chicago, Chicago, IL 60637, USA}

\author{Emre \"{O}z\"{u}lker}
\affiliation{Department of Physics, Istanbul Technical University, Maslak 34469 Istanbul, Turkey}

\author{Francesco Pace}
\affiliation{Dipartimento di Fisica, Universit\`a di Torino, Via P. Giuria 1, I-10125, Torino, Italy}
\affiliation{INFN, Sezione di Torino, Via P. Giuria 1, I-10125, Torino, Italy}

\author{Andronikos Paliathanasis}
\affiliation{Institute of Systems Science, Durban University of Technology, Durban 4000, South Africa}
\affiliation{Instituto de Ciencias F\'{\i}sicas y Matem\'{a}ticas, Universidad Austral de Chile, Valdivia, Chile}

\author{Antonella Palmese}
%\affiliation{NASA Einstein Fellow}
\affiliation{Department of Physics, University of California Berkeley, 366 LeConte Hall MC 7300, Berkeley, CA, 94720, USA}

\author{Supriya Pan}
\affiliation{Department of Mathematics, Presidency University, 86/1 College Street, Kolkata 700073, India}

\author{Daniela Paoletti}
\affiliation{Osservatorio di Astrofisica e Scienza dello Spazio di Bologna \& Istituto Nazionale di Astrofisica, via Gobetti 101, I-40129 Bologna, Italy}
\affiliation{INFN, Sezione di Bologna, viale Berti Pichat 6/2, 40127 Bologna, Italy}


\author{Santiago E. Perez Bergliaffa}
\affiliation{Departamento de F\'{\i}sica Te\'orica, Instituto de F\'{\i}sica, Universidade do Estado de Rio de Janeiro, CEP 20550-013, Rio de Janeiro, Brasil}


\author{Leandros Perivolaropoulos}
\affiliation{Department of Physics, University of Ioannina, GR-45110, Ioannina, Greece}

\author{Dominic~W.~Pesce}
\affiliation{Center for Astrophysics $|$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA 02138, USA}
\affiliation{Black Hole Initiative at Harvard University, 20 Garden Street, Cambridge, MA 02138, USA}

\author{Valeria Pettorino}
\affiliation{AIM, CEA, CNRS, Universit{\'e} Paris-Saclay, Universit{\'e} de Paris, F-91191 Gif-sur-Yvette, France}

\author{Oliver H.\,E. Philcox}
\affiliation{Department of Astrophysical Sciences, Princeton University, Princeton, NJ 08540, USA}%
\affiliation{School of Natural Sciences, Institute for Advanced Study, 1 Einstein Drive, Princeton, NJ 08540, USA}

\author{Levon Pogosian} 
\affiliation{Department of Physics, Simon Fraser University, Burnaby, BC, V5A 1S6, Canada}

\author{Vivian Poulin}
\affiliation{
 Laboratoire Univers \& Particules de Montpellier (LUPM), Universit\'e de Montpellier (UMR-5299) \\ Place Eug{\`e}ne Bataillon, F-34095 Montpellier Cedex 05, France 
}

\author{Gaspard Poulot}
\affiliation{School of Mathematics and Statistics, University of Sheffield, Hounsfield Road, Sheffield S3 7RH, United Kingdom}

\author{Marco Raveri}
\affiliation{Center for Particle Cosmology, Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}

\author{Mark J. Reid}
\affiliation{Harvard-Smithsonian Center for Astrophysics, 60 Garden Street, Cambridge, MA 02138, USA}

\author{Fabrizio Renzi}
\affiliation{Lorentz Institute for Theoretical Physics, Leiden University, PO Box 9506, Leiden 2300 RA, The Netherlands}

\author{Adam G. Riess}
\affiliation{Department of Physics and Astronomy, Johns Hopkins University, Baltimore, Maryland 21218, USA}

\author{Vivian I. Sabla}
\affiliation{Department of Physics \& Astronomy, Dartmouth College, 6127 Wilder Laboratory, Hanover, New Hampshire 03755 USA}

\author{Paolo Salucci}
\affiliation{SISSA, Via Bonomea 265, Trieste, 34100, Italy}
\affiliation{INFN, QGSKY Sez. Trieste, Italy}

\author{Vincenzo Salzano}
\affiliation{Institute of Physics, University of Szczecin, Wielkopolska 15, 70-451 Szczecin, Poland}

\author{Emmanuel N. Saridakis}
\affiliation{National Observatory of Athens, Lofos Nymfon, 11852 Athens, Greece}
\affiliation{Department of Astronomy, School of Physical Sciences, University of Science and Technology of China, Hefei, Anhui 230026, P.\ R.\ China} 
\affiliation{CAS Key Laboratory for Research in Galaxies and Cosmology,\\
University of Science and Technology of China, Hefei, Anhui 230026, China}


\author{Bangalore S. Sathyaprakash}
\affiliation{Institute for Gravitation and the Cosmos, Department of Physics,
Penn State University, University Park, Pennsylvania 16802, USA}
\affiliation{Department of Astronomy and Astrophysics, Penn State University, University Park, Pennsylvania 16802, USA} 
\affiliation{School of Physics and Astronomy, Cardiff University, Cardiff, CF24 3AA, United Kingdom}

\author{Martin Schmaltz}
\affiliation{Physics Department, Boston University, Boston, MA 02215, USA}

\author{Nils Sch\"oneberg}
\affiliation{Dept. F\'isica Qu\`antica i Astrof\'isica, Institut de Ci\`encies del Cosmos (ICCUB), Facultat de F\'isica, Universitat de Barcelona (IEEC-UB), Mart\'i i Franqu\'es, 1, E08028 Barcelona, Spain}

\author{Dan Scolnic}
\affiliation{Department of Physics, Duke University, Durham, NC 27708, USA}

\author{Anjan A. Sen}
\affiliation{School of Arts and Sciences, Ahmedabad University, Ahmedabad, Gujarat, India}
\affiliation{Centre for Theoretical Physics, Jamia Millia Islamia, New Delhi 110025, India}

\author{Neelima Sehgal}
\affiliation{Physics and Astronomy Department, Stony Brook University, Stony Brook, NY 11794, USA}

\author{Arman Shafieloo}
\affiliation{Korea Astronomy and Space Science Institute, Daejeon 34055, Korea}

\author{M.M. Sheikh-Jabbari}
\affiliation{ School of Physics, Institute for Research in Fundamental Sciences (IPM), P.O.Box 19395-5531, Tehran, Iran}

\author{Joseph Silk}
\affiliation{Institut d'Astrophysique, 75014 Paris, France}

\author{Alessandra Silvestri}
\affiliation{Lorentz Institute for Theoretical Physics, Leiden University, PO Box 9506, Leiden 2300 RA, The Netherlands}

\author{Foteini Skara}
\affiliation{Department of Physics, University of Ioannina, GR-45110, Ioannina, Greece}

\author{Martin S. Sloth}
\affiliation{CP$^3$-Origins, Center for Cosmology and Particle Physics Phenomenology, University of Southern Denmark, Campusvej 55, 5230 Odense M, Denmark}

\author{Marcelle Soares-Santos}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}

\author{Joan Sol\`a Peracaula}
\affiliation{Departament de F\'\i sica Qu\`antica i Astrof\'\i sica and Institute of Cosmos Sciences, Universitat de Barcelona, Av. Diagonal 647, E-08028 Barcelona, Catalonia, Spain}

\author{Yu-Yang Songsheng}
\affiliation{Key Laboratory for Particle Astrophysics, Institute of High Energy Physics, Chinese Academy of Sciences, 19B Yuquan Road, Beijing 100049, P.\ R.\ China}

\author{Jorge F. Soriano}
\affiliation{Department of Physics and Astronomy,  Lehman College, City University of New York, NY 10468, USA}
\affiliation{Department of Physics, Graduate Center, City University of New York,  NY 10016, USA}

\author{Denitsa Staicova}
\affiliation{Institute for Nuclear Research and Nuclear Energy, Bulgarian Academy of Sciences, Sofia 1784, Tsarigradsko shosse 72, Bulgaria}

\author{Glenn D. Starkman}
\affiliation{CERCA/ISO, Department of Physics, Case Western Reserve University, 10900 Euclid Avenue, Cleveland, OH 44106, USA}
\affiliation{Astrophysics Group \& Imperial Centre for Inference and Cosmology,
Department of Physics, Imperial College London, Blackett Laboratory,
Prince Consort Road, London SW7 2AZ, United Kingdom}

\author{Istv\'an Szapudi}
\affiliation{Institute for Astronomy, University of Hawaii, 2680 Woodlawn Drive, Honolulu, HI, 96822}

\author{Elsa M. Teixeira}
\affiliation{School of Mathematics and Statistics, University of Sheffield, Hounsfield Road, Sheffield S3 7RH, United Kingdom}


\author{Brooks Thomas}
\affiliation{Department of Physics, Lafayette College, Easton, PA 18042, USA}

\author{Tommaso Treu}
\affiliation{Department of Physics and Astronomy, University of California, Los Angeles CA 90095, USA}

\author{Emery Trott}
\affiliation{Department of Physics, University of Michigan, Ann Arbor, MI 48109, USA}

\author{Carsten van de Bruck}
\affiliation{School of Mathematics and Statistics, University of Sheffield, Hounsfield Road, Sheffield S3 7RH, United Kingdom}

\author{J. Alberto Vazquez}
\affiliation{Instituto de Ciencias F\'isicas, Universidad Nacional Aut\'onoma de M\'exico, Cuernavaca, Morelos, 62210, M\'exico}

\author{Licia Verde}
\affiliation{Institut de Ci\`encies del Cosmos, Universitat de Barcelona, Mart\'{\i} Franqu\`es 1, Barcelona 08028, Spain}
\affiliation{ICREA, Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats, Passeig Llu\'is Companys 23, Barcelona 08010, Spain}

\author{Luca Visinelli}
\affiliation{Tsung-Dao Lee Institute (TDLI) \& School of Physics and Astronomy, Shanghai Jiao Tong University, 
Shengrong Road 520, 201210 Shanghai, P.\ R.\ China}

\author{Deng Wang}
\affiliation{National Astronomical Observatories, Chinese Academy of Sciences, Beijing, 100012, P.\ R.\ China}

\author{Jian-Min Wang}
\affiliation{Key Laboratory for Particle Astrophysics, Institute of High Energy Physics, Chinese Academy of Sciences, 19B Yuquan Road, Beijing 100049, P.\ R.\ China}

\author{Shao-Jiang Wang}
\affiliation{CAS Key Laboratory of Theoretical Physics, Institute of Theoretical Physics, Chinese Academy of Sciences, Beijing 100190, P.\ R.\ China}

\author{Richard Watkins}
\affiliation{Department of Physics, Willamette University,
Salem, OR 97301, USA}
		
\author{Scott Watson}
\affiliation{Syracuse University, Syracuse, NY, USA}

\author{John K. Webb}
\affiliation{Clare Hall, University of Cambridge, Herschel Rd, Cambridge CB3 9AL, United Kingdom}

\author{Neal Weiner}
\affiliation{Center for Cosmology and Particle Physics, Department of Physics, New York University, New York, NY 10003, USA}

\author{Amanda Weltman}
\affiliation{HEPCAT Group, Department of Mathematics and Applied Mathematics,  University of Cape Town, South Africa, 7700}

\author{Samuel J. Witte}
\affiliation{Gravitation Astroparticle Physics Amsterdam (GRAPPA),
Anton Pannekoek Institute for Astronomy and Institute for Physics,
University of Amsterdam, Science Park 904, 1090 GL Amsterdam, The Netherlands}

\author{Rados\l{}aw Wojtak}
\affiliation{DARK, Niels Bohr Institute, University of Copenhagen, Jagtvej 128, 2200 Copenhagen, Denmark}

\author{Anil Kumar Yadav}
\affiliation{United College of Engineering and Research, Greater Noida - 201310, India} 

\author{Weiqiang Yang}
\affiliation{Department of Physics, Liaoning Normal University, Dalian, 116029, P.\ R.\ China}

\author{Gong-Bo Zhao}
\affiliation{National Astronomy Observatories, Chinese Academy of Sciences, Beijing, 100101, P.\ R.\ China}
\affiliation{University of Chinese Academy of Sciences, Beijing, 100049, P.\ R.\ China}

\author{Miguel Zumalac\'arregui}
\affiliation{Max Planck Institute for Gravitational Physics (Albert Einstein Institute),
Am M\"uhlenberg 1, D-14476 Potsdam-Golm, Germany}


